Formation Channels for Blue Straggler Stars

In this chapter we consider two formation channels for blue straggler stars: 1) the merger of two single stars via a collision, and 2) those produced via mass transfer within a binary. We review how computer simulations show that stellar collisions are likely to lead to relatively little mass loss and are thus effective in producing a young population of more-massive stars. The number of blue straggler stars produced by collisions will tend to increase with cluster mass. We review how the current population of blue straggler stars produced from primordial binaries decreases with increasing cluster mass. This is because exchange encounters with third, single stars in the most massive clusters tend to reduce the fraction of binaries containing a primary close to the current turn-off mass. Rather, their primaries tend to be somewhat more massive and have evolved off the main sequence, filling their Roche lobes in the past, often converting their secondaries into blue straggler stars (but more than 1 Gyr or so ago and thus they are no longer visible today as blue straggler stars).

==> common.tex <==
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\newcommand{\gras}[1]{\mbox{\boldmath $#1$}}
\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}          }\hbox{$\frown$}}}$}}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lapp{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\def\gapp{\ifmmode\stackrel{>}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}

\def\msol{\,\mathrm{M}_\odot}
\def\media#1{\langle #1\rangle}
\def\kms{~{\rm km~ s}^{-1}}
\def\sigp{\sigma_{\rm P}}


\def\aapr{A\&A Rev. }
\def\apjl{ApJL }
\def\aj{AJ }
\def\apj{ApJ }
\def\pasp{PASP }
\def\spie{SPIE }
\def\apjs{ApJS }
\def\araa{ARAA }
\def\aap{A\&A }
\def\mnras{MNRAS }
\def\nat{Nature }

\newcommand{\lesssim}    {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{<}}}}%
\newcommand{\lsim}       {\lesssim}%
\newcommand{\la}         {\lesssim}% For Springer A&A compliance...
\newcommand{\gtrsim}     {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{>}}}}%
\newcommand{\gsim}       {\gtrsim}%
\newcommand{\ga}         {\gtrsim}%
\newcommand{\sq}         {\mbox{\rlap{\ensuremath{\sqcap}}\ensuremath{\sqcup}}}%
\newcommand{\arcdeg}     {\mbox{\ensuremath{{}^\circ}}}%
\newcommand{\arcmin}     {\mbox{\ensuremath{{}^\prime}}}%
\newcommand{\arcsec}     {\mbox{\ensuremath{{}^{\prime\prime}}}}%

% Journal abbreviations
\def\aj{\rmfamily{AJ~}}           % Astronomical Journal
\def\apj{\rmfamily{ApJ~}}         % Astrophysical Journal
\def\apjl{\rmfamily{ApJ~}}        % Astrophysical Journal, Letters
\def\apjs{\rmfamily{ApJS~}}       % Astrophysical Journal, Supplement
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\aap{\rmfamily{A\&A~}}        % Astronomy and Astrophysics
\let\astap=\aap
\def\araa{\rmfamily{ARA\&A~}}     % Annual Review of Astronomy and Astrophysics
\def\aapr{\rmfamily{A\&A~Rev.~}}  % Astronomy and Astrophysics Reviews
\def\aaps{\rmfamily{A\&AS~}}      % Astronomy and Astrophysics, Supplement
\def\mnras{\rmfamily{MNRAS~}}     % Monthly Notices of the Royal Astron. Soc.
\def\pasp{\rmfamily{PASP~}}       % Publications of the Astron. Soc. o/t Pacific
\def\apss{\rmfamily{Ap\&SS~}}     % Astrophysics and Space Science
\def\pasj{\rmfamily{PASJ~}}       % Publications of the Astron. Soc. of Japan
\def\pra{\rmfamily{Phys.~Rev.~A~}}% Physical Review A: Atomic, Molecular, and  
                                  %   Optical Physics
\def\prb{\rmfamily{Phys.~Rev.~B~}}% Physical Review B: Condensed Matter and
                                  %   Materials Physics
\def\prc{\rmfamily{Phys.~Rev.~C~}}% Physical Review C: Nuclear Physics
\def\prd{\rmfamily{Phys.~Rev.~D~}}% Physical Review D: Particles, Fields,
                                  %   Gravitation and Cosmology
\def\pre{\rmfamily{Phys.~Rev.~E~}}% Physical Review E: Statistical, Nonlinear,
                                  %   and Soft Matter Physics
\def\rmp{\rmfamily{Rev.~Mod.~Phys.~}}% Reviews of Modern Physics
\def\prl{\rmfamily{Phys.~Rev.~Lett.~}}% Physical Review Letters
\def\nat{\rmfamily{Nature~}}      % Nature
\def\sci{\rmfamily{Science~}}     % Science
\def\skytel{\rmfamily{S\&T~}}     % Sky and Telescope
\def\ao{\rmfamily{Appl.~Opt.~}}   % Applied Optics
\let\applopt=\ao
\def\azh{\rmfamily{AZh~}}         % Astronomicheskii Zhurnal
\def\baas{\rmfamily{BAAS~}}       % Bulletin of the AAS
\def\jrasc{\rmfamily{JRASC~}}     % Journal of the Royal Astron. Soc. of Canada
\def\memras{\rmfamily{MmRAS~}}    % Memoirs of the Royal Astron. Soc.
\def\qjras{\rmfamily{QJRAS~}}     % Quarterly Journal of the Royal Astron. Soc.
\def\solphys{\rmfamily{Sol.~Phys.~}}% Solar Physics
\def\sovast{\rmfamily{Soviet~Ast.~}}% Soviet Astronomy
\def\ssr{\rmfamily{Space~Sci.~Rev.~}}% Space Science Reviews
\def\zap{\rmfamily{ZAp~}}         % Zeitschrift fuer Astrophysik
\def\iauc{\rmfamily{IAU~Circ.~}}  % IAU Cirulars
\let\iaucirc=\iauc
\def\aplett{\rmfamily{Astrophys.~Lett.~}}% Astrophysics Letters
\def\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.~}}% Astrophysics Space Physics
                                  % Research
\def\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands~}}% Bulletin of the 
                                  % Astronomical Institute of the Netherlands
\def\fcp{\rmfamily{Fund.~Cosmic~Phys.~}}% Fundamental Cosmic Physics
\def\gca{\rmfamily{Geochim.~Cosmochim.~Acta~}}% Geochimica Cosmochimica Acta
\def\grl{\rmfamily{Geophys.~Res.~Lett.~}}% Geophysics Research Letters
\def\jcp{\rmfamily{J.~Chem.~Phys.~}}% Journal of Chemical Physics
\def\jgr{\rmfamily{J.~Geophys.~Res.~}}% Journal of Geophysics Research
\def\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.~}} % Journal of Quantitative
                                  % Spectroscopy and Radiative Transfer
\def\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana~}}
                                  % Mem. Societa Astronomica Italiana
\def\nphysa{\rmfamily{Nucl.~Phys.~A~}}% Nuclear Physics A
\def\physrep{\rmfamily{Phys.~Rep.~}}% Physics Reports
\def\physscr{\rmfamily{Phys.~Scr~}}% Physica Scripta
\def\planss{\rmfamily{Planet.~Space~Sci.~}}% Planetary Space Science
\def\procspie{\rmfamily{Proc.~SPIE~}}% Proceedings of the SPIE
\def\aipconf{\rmfamily{AIP~Conf.~Proc.~}}% AIP Conference Proceedings
\def\aspconf{\rmfamily{ASP~Conf.~Ser.~}}% ASP Conference Series
\def\asslconf{\rmfamily{Ap\&SSL~Conf.~Ser.~}}% ASSL Conference Series}
\def\maps{\rmfamily{MAPS~}}       % Meteoritics and Planetary Science

\usepackage{amsmath}
\usepackage{amssymb}

\def\Teff{$T_{\rm eff}$}
\def\Msun{{\rm M}_\odot}
\def\Rsun{{\rm R}_\odot}
\def\kms{\rm km~s$^{-1}$}

\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}                         }\hbox{$\frown$}}}$}}

\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}


\newcommand{\half}{{\ensuremath{\textstyle\frac12}}}
\newcommand{\threehalf}{{\ensuremath{\textstyle\frac32}}}
\newcommand{\third}{{\ensuremath{\textstyle\frac13}}}
\newcommand{\quarter}{{\ensuremath{\textstyle\frac14}}}
\newcommand\apgt{\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand\aplt{\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\newcommand{\kin}{{\ensuremath K}}
\newcommand{\mbar}{{\ensuremath \langle m\rangle}}
\newcommand{\msun}{{\ensuremath M_\odot}}
\newcommand{\pot}{{\ensuremath U}}
\newcommand{\rvir}{{\ensuremath R_{vir}}}
\newcommand{\rh}{{\ensuremath R_h}}
\newcommand{\rj}{{\ensuremath R_J}}
\newcommand{\rsun}{{\ensuremath R_\odot}}
\newcommand{\tcc}{{\ensuremath t_{cc}}}
\newcommand{\tdis}{{\ensuremath t_{dis}}}
\newcommand{\tdyn}{{\ensuremath t_{dyn}}}
\newcommand{\tr}{{\ensuremath t_r}}
\newcommand{\tenc}{{\ensuremath t_{enc}}}
\newcommand{\trh}{{\ensuremath t_{rh}}}
\newcommand{\trl}{{\ensuremath t_{rl}}}
\newcommand{\tseg}{{\ensuremath t_{seg}}}
\newcommand{\vdisp}{{\ensuremath \langle v^2\rangle}}
\newcommand{\vrms}{{\ensuremath \vdisp^{1/2}}}
\newcommand{\vesc}{{\ensuremath v_{esc}}}
\newcommand{\vinf}{{\ensuremath v_\infty}}

\newcommand{\vv}{{\bf v}}
\newcommand{\vx}{{\bf x}}
\newcommand{\va}{{\bf a}}





